Thermodynamic Uncertainty Relations for Steady-State Thermodynamics

A system can be driven out of equilibrium by both time-dependent and nonconservative forces, which gives rise to a decomposition of the dissipation into two non-negative components, called the excess and housekeeping entropy productions. We derive thermodynamic uncertainty relations for the excess and housekeeping entropy. These can be used as tools to estimate the individual components, which are in general difficult to measure directly. We introduce a decomposition of an arbitrary current into excess and housekeeping parts, which provide lower bounds on the respective entropy production. Furthermore, we also provide a geometric interpretation of the decomposition, and show that the uncertainties of the two components are not independent, but rather have to obey a joint uncertainty relation, which also yields a tighter bound on the total entropy production. We apply our results to two examples that illustrate the physical interpretation of the components of the current and how to estimate the entropy production.

==> HS_TUR(arXiv)/commands.tex <==
%=============== 独自定義マクロ=====================
\newcommand{\expo}{\mathrm{e}}
\newcommand{\pdif}[2]{\frac{\partial #1}{\partial #2}}%偏微分
\newcommand{\ppdif}[2]{\frac{\partial^2 #1}{\partial #2^2}}%２階偏微分
\newcommand{\dif}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}}%微分
\newcommand{\ddif}[2]{\frac{\mathrm{d}^2 #1}{\mathrm{d} #2^2}}%２階微分
\newcommand{\eqdef}{\ensuremath{\stackrel{\mathrm{def}}{=}}}
\newcommand{\eqexcl}{\ensuremath{\stackrel{!}{=}}}
\newcommand{\eqhat}{\ensuremath{\widehat{=}}}
\newcommand{\ii}{\mathrm{i}}
\newcommand{\jj}{\mathrm{j}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\sh}{\mathrm{shell}}
\newcommand{\bd}{\bar{D}}
\newcommand{\aee}{\bar{\mathbf{\varepsilon}}}
\newcommand{\am}{\bar{\mathbf{\mu}}}
\newcommand{\aii}{\bar{\mathsf{I}}}
\newcommand{\acc}{\bar{\mathbf{\chi}}}
\newcommand{\ozz}{\omega_{0}}
\newcommand{\omm}{\omega_{M}}
%\newcommand{\hami}{\hat{H}}
%\newcommand{\dens}{\hat{\rho}}
%\newcommand{\obs}{\hat{O}}%オブザーバブル
\newcommand{\trace}[2][]{\operatorname{Tr}_{#1}\left(#2\right)}
\newcommand{\vca}[1]{\overrightarrow{#1}}

\newcommand{\hami}{{H}}
\newcommand{\dens}{{\rho}}
\newcommand{\obs}{{O}}%オブザーバブル



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% equation %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\eq}[1]{\begin{equation} #1 \end{equation}}
%\newcommand{\eqa}[2]{\begin{equation} #1 \label{eq:#2} \end{equation}}
%\newcommand{\balign}[1]{\begin{align} #1 \end{align}}
%\newcommand{\bcases}[1]{\begin{cases} #1 \end{cases}}
%\newcommand{\beqary}[1]{\begin{eqnarray}#1 \end{eqnarray}}
%\newcommand{\mx}[1]{\begin{pmatrix}#1 \end{pmatrix}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%Style and such%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dis}{\displaystyle}
\newcommand{\txt}{\textstyle}
\newcommand{\bs}{\boldsymbol}
\newcommand{\ul}{\ulinej}
\newcommand{\fn}{\footnote}
\newcommand{\fnm}{\footnotemark}
\newcommand{\fnt}{\footnotetext}

\newcommand{\bitem}[2]{\begin{itembox}[l]{#1} #2 \end{itembox}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Basic symbol 1 %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


\newcommand{\figin}[4]
{\begin{figure}[tb]
\centering
\includegraphics[width= #1]{#2.pdf}
\caption{#3}
\label{fig:#4}
\end{figure}}

\newcommand{\figinb}[4]
{
\erase{
\begin{figure}[t]\centering\includegraphics[width= #1]{#2}\caption{#3}\label{f:#4}\end{figure}
}
}

\newcommand{\todayd}{\the\year/\the\month/\the\day}
\newcommand{\del}{\partial}
%\newcommand{\ep}{\epsilon}
\newcommand{\bib}{\bibitem}
\newcommand{\appnum}[1]{\renewcommand{\theequation}{#1.\arabic{equation} }
\setcounter{equation}{0}}


\newcommand{\Ima}{\operatorname{Im}}
\newcommand{\up}{\uparrow}
\newcommand{\down}{\downarrow}
\newcommand{\mr}{\mathrm}
\newcommand{\lr}{\leftrightarrow}
\newcommand{\const}{\mathrm{const}}
\newcommand{\lmd}{\lambda}
\newcommand{\Lmd}{\Lambda}
\newcommand{\ssk}{\shortstack}
\newcommand{\lb}{\label}
\newcommand{\nt}{\notag}% no number of equation
\newcommand{\Tr}{\operatorname{Tr}}
\newcommand{\ft}[2]{\left. #1 \right|_{#2}}




\newcommand{\blist}[2]{\begin{easylist}[#1] #2 \end{easylist}}
\newcommand{\bel}{\begin{easylist}}
\newcommand{\eel}{\end{easylist}}
%http://id.fnshr.info/2014/01/04/easylist/
\newcommand{\bi}[1]{\begin{itemize} #1 \end{itemize}}
\newcommand{\be}[1]{\begin{enumerate} #1 \end{enumerate}}


\newcommand{\eref}[1]{Eq.~\eqref{#1}}
\newcommand{\tref}[1]{Thm.~\ref{#1}}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\sref}[1]{Sec.~\ref{#1}}
\newcommand{\ccite}[1]{Ref.~\cite{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   brackets and such
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\lef}{\left(}
\newcommand{\rig}{\right)}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
%%%%%%%%%%%%
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\norms}[1]{\Vert#1\Vert}
\newcommand{\normi}[1]{\bigl\Vert#1\bigr\Vert_\infty}
\newcommand{\rbk}[1]{\left(#1\right)}
\newcommand{\srbk}[1]{(#1)}
\newcommand{\sqbk}[1]{\left[#1\right]}
\newcommand{\cbk}[1]{\left\{#1\right\}}
\newcommand{\bkt}[1]{\left\langle#1\right\rangle}
\newcommand{\sbkt}[1]{\langle#1\rangle}
\newcommand{\bbkt}[1]{\bigl\langle#1\bigr\rangle}
%\newcommand{\set}[2]{\left\{#1\,\Bigl|\,#2\right\}}
\newcommand{\rvbar}[1]{\left.#1\right|}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   special sums and such
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sumtwo}[2]%
{\mathop{\sum_{#1}}_{#2}}
\newcommand{\sumthree}[3]%
{\mathop{\mathop{\sum_{#1}}_{#2}}_{#3}}
\newcommand{\sumfour}[4]%
{\mathop{\mathop{\mathop{\sum_{#1}}_{#2}}_{#3}}_{#4}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\prodtwo}[2]%
{\mathop{\prod_{#1}}_{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mintwo}[2]%
{\mathop{\min_{#1}}_{#2}}
\newcommand{\maxtwo}[2]%
{\mathop{\max_{#1}}_{#2}}
\newcommand{\maxthree}[3]%
{\mathop{\mathop{\max_{#1}}_{#2}}_{#3}}
\newcommand{\limtwo}[2]%
{\mathop{\lim_{#1}}_{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\suptwo}[2]%
{\mathop{\sup_{#1}}_{#2}}
\newcommand{\supthree}[3]%
{\mathop{\mathop{\sup_{#1}}_{#2}}_{#3}}
\newcommand{\supfour}[4]%
{\mathop{\mathop{\mathop{\sup_{#1}}_{#2}}_{#3}}_{#4}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\inftwo}[2]%
{\mathop{\inf_{#1}}_{#2}}
\newcommand{\infthree}[3]%
{\mathop{\mathop{\inf_{#1}}_{#2}}_{#3}}
\newcommand{\inffour}[4]%
{\mathop{\mathop{\mathop{\inf_{#1}}_{#2}}_{#3}}_{#4}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   Caligraphic letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\calA{{\mathcal A}}
\newcommand\calB{{\mathcal B}}
\newcommand\calC{{\mathcal C}}
\newcommand\calD{{\mathcal D}}
\newcommand\calE{{\mathcal E}}
\newcommand\calF{{\mathcal F}}
\newcommand\calG{{\mathcal G}}
\newcommand\calH{{\mathcal H}}
\newcommand\calI{{\mathcal I}}
\newcommand\calJ{{\mathcal J}}
\newcommand\calK{{\mathcal K}}
\newcommand\calL{{\mathcal L}}
\newcommand\calM{{\mathcal M}}
\newcommand\calN{{\mathcal N}}
\newcommand\calO{{\mathcal O}}
\newcommand\calP{{\mathcal P}}
\newcommand\calQ{{\mathcal Q}}
\newcommand\calR{{\mathcal R}}
\newcommand\calS{{\mathcal S}}
\newcommand\calT{{\mathcal T}}
\newcommand\calU{{\mathcal U}}
\newcommand\calV{{\mathcal V}}
\newcommand\calW{{\mathcal W}}
\newcommand\calX{{\mathcal X}}
\newcommand\calY{{\mathcal Y}}
\newcommand\calZ{{\mathcal Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tid}{\tilde{d}}
\newcommand{\tis}{\tilde{s}}
\newcommand{\tiv}{\tilde{v}}
\newcommand{\tix}{\tilde{x}}
\newcommand{\tiy}{\tilde{y}}
\newcommand{\tiz}{\tilde{z}}
\newcommand{\tiS}{\tilde{S}}
\newcommand{\tidelta}{\tilde{\delta}}
\newcommand{\tipsi}{\tilde{\psi}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mrO}{\mathrm{O}}
\newcommand{\mrP}{\mathrm{P}}
\newcommand{\mrQ}{\mathrm{Q}}
\newcommand{\mrR}{\mathrm{R}}
\newcommand{\mrS}{\mathrm{S}}
\newcommand{\mrr}{\mathrm{r}}
\newcommand{\mrx}{\mathrm{x}}
\newcommand{\mry}{\mathrm{y}}
\newcommand{\mrz}{\mathrm{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% BOLD SYMBOL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bsa}{\boldsymbol{a}}
\newcommand{\bsb}{\boldsymbol{b}}
\newcommand{\bsc}{\boldsymbol{c}}
\newcommand{\bsd}{\boldsymbol{d}}
\newcommand{\bse}{\boldsymbol{e}}
\newcommand{\bsf}{\boldsymbol{f}}
\newcommand{\bsg}{\boldsymbol{g}}
\newcommand{\bsh}{\boldsymbol{h}}
\newcommand{\bsi}{\boldsymbol{i}}
\newcommand{\bsj}{\boldsymbol{j}}
\newcommand{\bsk}{\boldsymbol{k}}
\newcommand{\bsl}{\boldsymbol{l}}
\newcommand{\bsm}{\boldsymbol{m}}
\newcommand{\bsn}{\boldsymbol{n}}
\newcommand{\bso}{\boldsymbol{o}}
\newcommand{\bsp}{\boldsymbol{p}}
\newcommand{\bsq}{\boldsymbol{q}}
\newcommand{\bsr}{\boldsymbol{r}}
\newcommand{\bss}{\boldsymbol{s}}
\newcommand{\bst}{\boldsymbol{t}}
\newcommand{\bsu}{\boldsymbol{u}}
\newcommand{\bsv}{\boldsymbol{v}}
\newcommand{\bsw}{\boldsymbol{w}}
\newcommand{\bsx}{\boldsymbol{x}}
\newcommand{\bsy}{\boldsymbol{y}}
\newcommand{\bsz}{\boldsymbol{z}}
%%%%%%%%%%%%
\newcommand{\bsA}{\boldsymbol{A}}
\newcommand{\bsB}{\boldsymbol{B}}
\newcommand{\bsC}{\boldsymbol{C}}
\newcommand{\bsD}{\boldsymbol{D}}
\newcommand{\bsE}{\boldsymbol{E}}
\newcommand{\bsF}{\boldsymbol{F}}
\newcommand{\bsG}{\boldsymbol{G}}
\newcommand{\bsH}{\boldsymbol{H}}
\newcommand{\bsI}{\boldsymbol{I}}
\newcommand{\bsJ}{\boldsymbol{J}}
\newcommand{\bsK}{\boldsymbol{K}}
\newcommand{\bsL}{\boldsymbol{L}}
\newcommand{\bsR}{\boldsymbol{R}}
\newcommand{\bsS}{\boldsymbol{S}}
\newcommand{\bsU}{\boldsymbol{U}}
\newcommand{\bsV}{\boldsymbol{V}}
%%%%%%%%%%%%
\newcommand{\bszero}{\boldsymbol{0}}
%%%%%%%%%%%%
\newcommand{\bsalpha}{\boldsymbol{\alpha}}
\newcommand{\bsdelta}{\boldsymbol{\delta}}
\newcommand{\bsell}{\boldsymbol{\ell}}
\newcommand{\bsth}{\boldsymbol{\theta}}
\newcommand{\bsxi}{\boldsymbol{\xi}}
\newcommand{\bsrho}{\boldsymbol{\rho}}
%%%%%%%%%%%%
\newcommand{\bsPsi}{\boldsymbol{\Psi}}
\newcommand{\bsOmega}{\boldsymbol{\Omega}}
%%%%%%%%%%%%
\newcommand{\bsna}{\boldsymbol{\nabla}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}
\newcommand{\unitmatrix}{\mathsf{I}}
\newcommand{\zeromatrix}{\mathsf{0}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbZ}{\mathbb{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   Frequently used symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ep}{\varepsilon}
\newcommand{\dn}{\downarrow}
\newcommand{\bcs}{\backslash}
\newcommand{\Di}{\mathit{\Delta}}
\newcommand{\qedm}{\rule{1.5mm}{3mm}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\para}[1]{{\em #1}\/.---}
\newcommand{\ns}[1]{\textbf{[NS: #1]}}
\newcommand{\tm}[1]{\textbf{[TM: #1]}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%This paper
\newcommand{\tot}{\mathrm{tot}}
\newcommand{\hk}{\mathrm{hk}}
\newcommand{\ex}{\mathrm{ex}}
\newcommand{\ssrm}{\mathrm{ss}}
%\newcommand{\eqrm}{\mathrm{eq}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\vct}[1]{\bm{#1}}
